Exploiting Partial Order of Keys to Verify Security of a Vehicular Group Protocol

Vehicular networks will enable a range of novel applications to enhance road traffic efficiency, safety, and reduce fuel consumption. As for other cyber-physical systems, security is essential to the deployment of these applications and standardisation efforts are ongoing. In this paper, we perform a systematic security evaluation of a vehicular platooning protocol through a thorough analysis of the protocol and security standards. We tackle the complexity of the resulting model with a proof strategy based on a relation on keys. The key relation forms a partial order, which encapsulates both secrecy and authenticity dependencies. We show that our order-aware approach makes the verification feasible and proves strong authenticity properties along with secrecy of all keys used throughout the protocol.

==> header.tex <==
%%%% PACKAGES %%%%%%%%%%%%%%
% SYMBOLS
\usepackage{latexsym,amsfonts,amsmath,amssymb,amsthm}
\usepackage{xspace}
\usepackage{enumitem}           % mainly for (i),(ii) in enumerate env.

% ENV
\usepackage[strict]{changepage} % for adjustwidth environment
\usepackage{framed} % for formal definitions

% FIGURES
\usepackage{msc}
\usepackage{anb}
\usepackage{booktabs}           % better tabular
\usepackage[most]{tcolorbox}    % for tcolorbox

% EDITORIAL
\usepackage{todonotes}
\usepackage{pdfcomment}

% OTHERS
\usepackage{cleveref}


%%%% ENVIRONMENTS %%%%%%%%%%%%%%
% environment derived from framed.sty: see leftbar environment definition
\definecolor{formalshade}{rgb}{0.95,0.95,1}
\definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}
\newenvironment{formal}{%
\def\FrameCommand{%
\hspace{1pt}%
{\color{darkblue}\vrule width 2pt}%
{\color{formalshade}\vrule width 4pt}%
\colorbox{formalshade}%
}%
\MakeFramed{\advance\hsize-\width\FrameRestore}%
\noindent\hspace{-4.55pt}% disable indenting first paragraph
\begin{adjustwidth}{}{7pt}%
\vspace{2pt}\vspace{2pt}%
}
{%
\vspace{2pt}\end{adjustwidth}\endMakeFramed%
}

==> key_hierarchy.tex <==
\tikzset{
  basic/.style  = {draw, text width=2cm, drop shadow, font=\sffamily, rectangle},
  root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=white},
  level-2/.style = {basic, rounded corners=6pt, thin,align=center, fill=white, text width=2.5cm},
  level-3/.style = {basic, thin, align=center, fill=white, text width=2.4cm}
}

%one box per key
%different arrows for secrecy/ (forgeability/authentication)

\begin{figure}[H]
    \centering
\begin{tikzpicture}[
  level 1/.style={sibling distance=10em, level distance=5em},
%   {edge from parent fork down},
  edge from parent/.style={->,solid,black,thick,sloped,draw}, 
  edge from parent path={(\tikzparentnode.south) -- (\tikzchildnode.north)},
  >=latex, node distance=1cm, edge from parent fork down]



% The second level, relatively positioned nodes
\begin{scope}[every node/.style={root}]
\node (ltkCA) {$ltk_{CA}$};



\node [below left = 8mm and 10mm of ltkCA.east, text width = 15mm] (c2) {$ltk_2$};
\draw[->, dashed] (c2) -- (ltkCA);

\node [left = 5mm of c2, text width = 15mm]  (c1) {$ltk_1$};
\draw[->, dashed] (c1) -- (ltkCA);

\node [right = 5mm of c2, text width = 15mm] (c3) {$ltk_3$};
\draw[->, dashed] (c3) -- (ltkCA);

\node [right = 5mm of c3, text width = 15mm] (cn) {$ltk_n$};
\draw[->, dashed] (cn) -- (ltkCA);





\node [below left = 8mm and 5mm of c2.east, text width = 15mm] (c21) {$jrek_2$};

\node [below left = 10mm and 14 mm of c21.east, text width = 20mm ] (c11) {$eJoin_{1}$};
\draw[->, dashed] (c11) -- (c1);


\draw[->, dashed] (c21) -- (c2);
\draw[->] (c11) -- (c21.south);


\node [below left = 8mm and 5mm of c3.east, text width = 15mm] (c31) {$jrek_3$};
\draw[->, dashed] (c31) -- (c3);

\node [right = 5mm of c31, text width = 15mm] (c3n) {$jrek_n$};
\draw[->, dashed] (c3n) -- (cn);

\node [right = 12mm of c11,  text width = 20mm] (c32) {$eJoin_{2}$};
\draw[->] (c32) -- (c31.south);
\draw[->, dashed] (c32) -- (c2);

\node [right = 3mm of c32,  text width = 22mm] (c33) {$eJoin_{n-1}$};
\draw[->] (c33) -- (c3n.south);
\draw[->, dashed] (c33) -- (c3);

\node [below = 8mm of c11, text width = 10mm ] (c41) {$ppk_{1}$};

\node [right = 8mm of c41, text width = 10mm ] (c42) {$ppk_{2}$};

\node [below = 8mm of c33, text width = 10mm ] (c43) {$ppk_{n}$};


\draw[->] (c41) -- (c11.south);
\draw[->] (c42) -- (c32.south);
\draw[->] (c43) -- (c33.south);

\node [ text width = 10mm ] (c51) at ($(c42)!0.5!(c43)$) {$pgk$};

\draw[->] (c51) -- (c11.south);
\draw[->] (c51) -- (c32.south);
\draw[->] (c51) -- (c33.south);


\node [below = 8mm of c41, text width = 15mm ] (c63) {$eKupdate$};
\draw[->] (c63) -- (c41.south);

\node [right = 30mm of c63, text width = 13mm ] (c61) {$eLeave$};
\draw[->] (c61) -- (c51.south);

\node [right = 5mm of c61, text width = 12mm ] (c62) {$eKUR$};
\draw[->] (c62) -- (c51.south);

\node [right = 5mm of c63, text width = 18mm ] (c71) {$pgkUpdate$};
\draw[->] (c71) -- (c63.east);
%\draw[->] (c71) -- (c42.south);

\end{scope}

% lines from each level 1 node to every one of its "children"
%\foreach \value in {1,2,3}
%  \draw[->] (c1.195) |- (c1\value.west);

%\foreach \value in {1,2,3}
%  \draw[->] (c1) |- (c1\value.north);

%\foreach \value in {1,...,4}
%  \draw[->] (c2.195) |- (c2\value.west);

%\foreach \value in {1,...,5}
%  \draw[->] (c3.195) |- (c3\value.west);
  

\end{tikzpicture}
    \caption{Illustration of partial order of keys in Ensemble. Dashed arrows illustrate authentication dependencies and solid arrows illustrate secrecy dependencies. We have omitted transitive arrows and self loops, as well as overlapping arrows. Subscripts for \textit{jrek} and \textit{eJoin} have been added to differentiate the instances from distinct message exchanges.}
    \label{fig:hierarchy}
\end{figure}




==> old_protocol_diagram.tex <==
%\input{header}
\input{macros}


\definecolor{gris}{gray}{0.85}
\begin{figure*}[t]
  \centering
  \setmsckeyword{}
  \drawframe{no}    % uncomment to not draw a frame
  \begin{msc}[
    /msc/title top distance=0cm,
    /msc/first level height=.2cm,
    /msc/last level height=0.4cm,
    /msc/head height=0cm,
    /msc/instance width=0cm,
    /msc/head top distance=0.5cm,
    /msc/foot distance=-0.0cm,
    /msc/instance width=0cm,
    /msc/condition height=0.2cm
    ]
    {}
    %%%%%%%%%%%%%%%%%% CONFIG %%%%%%%%%%%%%%%%%%%%%%%%%
    \setlength{\instwidth}{0\mscunit} % to remove default box below agents 
    \setlength{\instdist}{6cm}  % defalut value between agent
    % \setlength{\regionbarwidth}{0\mscunit}
    % \setlength{\instfootheight}{0\mscunit}
    % \setlength{\instheadheight}{.5\mscunit}
    % \setlength{\bottomfootdist}{0\mscunit}

    %%%%%%%%%%%%%%%%%% AGENTS %%%%%%%%%%%%%%%%%%%%%%%%%
   \declinst{A}{             
    Vehicle 1
    }{}
    \declinst{B}{             
    Vehicle 2
    }{}
    \declinst{C}{             
    Vehicle 3
    }{}
    
    \nextlevel[0.5]
    
        %%%%%%%%%%%%%%%%%% ACTIONS %%%%%%%%%%%%%%%%%%%%%%%%%
    %%% AUTH TOKEN ---> SN ---> UE
    \action*{\parbox{4cm}{\scriptsize{$
          \begin{array}[c]{l}
            \APP\leftarrow \CAM, \joinable \\
            \GN\leftarrow \APP, \sign(\APP, \ltkA), \certA 
          \end{array}
          $}}}{A}

\nextlevel[2.8]
    
    \mess{\messLabel{Cooperative Awareness Message}}{A}{B}
    
    \nextlevel[0.8]
    
    %%% RESPONSE UE --> SN
    \action*{\parbox{4cm}{\scriptsize{$
          \begin{array}[c]{l}
           \mathsf{generate~key-pair}\ \jrekA, \pkjrekA \\
           \APP\leftarrow \JR, \pkjrekA \\
           \GN\leftarrow \APP, \sign(\APP, \ltkB), \certB 
          \end{array}
          $}}}{B}
    \nextlevel[3]
    %\nextlevel[2]
    
    \mess{\messLabel{Join Request}}{B}{A}
    
\nextlevel[0.7]

%  rekRecipInfo = <h(pk(~jrekBA)), aenc(~ephemeralAB, pk(~jrekBA))>
%  ciphertext = <senc(<~ppkAB, ~pgk>, ~ephemeralAB)>
%  app = <'JRE', rekRecipInfo, ciphertext, $B>
%  cert = <$A, pk(~ltkA), sigCA>
%  gn = <app, sign(app, ~ltkA), cert>
  
    \action*{\parbox{6.5cm}{\scriptsize{$
          \begin{array}[c]{l}
            \mathsf{generate~keys}\ \ejoinA, \ppkA, \pgk \\
           \rekRecipInfo\leftarrow h(\pkjrekA), \aenc(\ejoinA, \pkjrekA) \\
           \ciphertext\leftarrow \senc(\tuple{\ppkA, \pgk}, \ejoinA)\\
           \APP\leftarrow \JRE, \rekRecipInfo, \ciphertext, \idB \\
           \GN\leftarrow \APP, \sign(\APP, \ltkA), \certA 
          \end{array}
          $}}}{A}
    \nextlevel[5]
    
    \mess{\messLabel{Join Response}}{A}{B}

    \nextlevel[0.4]
    \condition{Agreement on $\ppkA$, $\pgk$}{A,B}
    \nextlevel[1.7]
    
        \action*{\parbox{4cm}{\scriptsize{$
          \begin{array}[c]{l}
            \APP\leftarrow \CAM, \joinable \\
            \GN\leftarrow \APP, \sign(\APP, \ltkB), \certB
          \end{array}
          $}}}{B}

\nextlevel[3]


    \mess{\messLabel{Cooperative Awareness Message}}{B}{C}
    
    \nextlevel[0.5]
    
    %%% RESPONSE UE --> SN
    \action*{\parbox{4cm}{\scriptsize{$
          \begin{array}[c]{l}
           \mathsf{generate~key-pair}\ \jrekB, \pkjrekB \\
           \APP\leftarrow \JR, \pkjrekB \\
           \GN\leftarrow \APP, \sign(\APP, \ltkB), \certB 
          \end{array}
          $}}}{C}
          
    \nextlevel[3]
    
    \mess{\messLabel{Join Request}}{C}{B}
    
\nextlevel[0.5]

%  rekRecipInfo = <h(pk(~jrekBA)), aenc(~ephemeralAB, pk(~jrekBA))>
%  ciphertext = <senc(<~ppkAB, ~pgk>, ~ephemeralAB)>
%  app = <'JRE', rekRecipInfo, ciphertext, $B>
%  cert = <$A, pk(~ltkA), sigCA>
%  gn = <app, sign(app, ~ltkA), cert>
  
    \action*{\parbox{6.5cm}{\scriptsize{$
          \begin{array}[c]{l}
            \mathsf{generate~keys}\ \ejoinA, \ppkA, \pgk \\
           \rekRecipInfo\leftarrow h(\pkjrekA), \aenc(\ejoinA, \pkjrekA) \\
           \ciphertext\leftarrow \senc(\tuple{\ppkA, \pgk}, \ejoinA)\\
           \APP\leftarrow \JRE, \rekRecipInfo, \ciphertext, \idB \\
           \GN\leftarrow \APP, \sign(\APP, \ltkA), \certA 
          \end{array}
          $}}}{B}
    \nextlevel[5]
    
    \mess{\messLabel{Join Response}}{B}{C}

   \nextlevel[0.4]
    \condition{Agreement on $\ppkB$, $\pgk$}{B,C}
    \nextlevel[1.7]
    
\action*{\parbox{4cm}{\scriptsize{$
          \begin{array}[c]{l}
            \APP\leftarrow \CAM, \joinable \\
            \GN\leftarrow \APP, \sign(\APP, \ltkB), \certB
          \end{array}
          $}}}{C}
   \nextlevel[2.3]
    
    \mess{\messLabel{Leave}}{C}{B}

    \nextlevel[0.5]
    
\action*{\parbox{4cm}{\scriptsize{$
          \begin{array}[c]{l}
            \APP\leftarrow \CAM, \joinable \\
            \GN\leftarrow \APP, \sign(\APP, \ltkB), \certB
          \end{array}
          $}}}{B}
   \nextlevel[3]
    
    \mess{\messLabel{Key Update Request}}{B}{A}
    
        \nextlevel[0.5]
    
\action*{\parbox{4cm}{\scriptsize{$
          \begin{array}[c]{l}
            \APP\leftarrow \CAM, \joinable \\
            \GN\leftarrow \APP, \sign(\APP, \ltkB), \certB
          \end{array}
          $}}}{A}
   \nextlevel[2]
    
    \mess{\messLabel{Key Update}}{A}{B}
    
    \nextlevel[0.5]
    \condition{Agreement on $\pgkUpdate$}{A,B}
    \nextlevel[1.7]

  \end{msc}
  \vspace{-10pt}
  \caption{The modeled ENSEMBLE protocol interactions}
  \label{fig:EAP-AKAp}
\end{figure*}


==> plot_data/plotcomm <==
set terminal pdf enhanced size 8cm, 6cm
set output 'time.pdf'
set style data lines
set xrange [10:12000]
set yrange [0:31]
set xlabel "Time (s)"
set logscale x
set ylabel "Verified lemmas (out of 19)"
plot  "< sort -nk17 -t \" \" results.txt" using ($17):($0) lw 3 title "Order-aware" with steps,\
      "< sort -nk13 -t \" \" results.txt" using ($13):($0) lw 3 title "Oracle only" with steps, \
      "< sort -nk9 -t \" \" results.txt" using ($9):($0) lw 3 title "Lemma reuse" with steps, \
      "< sort -nk5 -t \" \" results.txt" using ($5):($0) lw 3 title "Bare Tamarin" with steps

pause -1
